Three Ehrhart Quasi-polynomials

Let $P(b)\subset R^d$ be a semi-rational parametric polytope, where $b=(b_j)\in R^N$ is a real multi-parameter. We study intermediate sums of polynomial functions $h(x)$ on $P(b)$, $$ S^L (P(b),h)=\sum_{y}\int_{P(b)\cap (y+L)} h(x) \mathrm dx, $$ where we integrate over the intersections of $P(b)$ with the subspaces parallel to a fixed rational subspace $L$ through all lattice points, and sum the integrals. The purely discrete sum is of course a particular case ($L=0$), so $S^0(P(b), 1)$ counts the integer points in the parametric polytopes. The chambers are the open conical subsets of $R^N$ such that the shape of $P(b)$ does not change when $b$ runs over a chamber. We first prove that on every chamber of $R^N$, $S^L (P(b),h)$ is given by a quasi-polynomial function of $b\in R^N$. A key point of our paper is an analysis of the interplay between two notions of degree on quasi-polynomials: the usual polynomial degree and a filtration, called the local degree. Then, for a fixed $k\leq d$, we consider a particular linear combination of such intermediate weighted sums, which was introduced by Barvinok in order to compute efficiently the $k+1$ highest coefficients of the Ehrhart quasi-polynomial which gives the number of points of a dilated rational polytope. Thus, for each chamber, we obtain a quasi-polynomial function of $b$, which we call Barvinok's patched quasi-polynomial (at codimension level $k$). Finally, for each chamber, we introduce a new quasi-polynomial function of $b$, the cone-by-cone patched quasi-polynomial (at codimension level $k$), defined in a refined way by linear combinations of intermediate generating functions for the cones at vertices of $P(b)$. We prove that both patched quasi-polynomials agree with the discrete weighted sum $b\mapsto S^0(P(b),h)$ in the terms corresponding to the $k+1$ highest polynomial degrees.

==> Makefile <==
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=3-Ehrhart-polynomials-arXiv

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

THREEPOLY_GRAPHICS_SOURCES=

THREEPOLY_GENERATED_GRAPHICS=$(THREEPOLY_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(THREEPOLY_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(THREEPOLY_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(THREEPOLY_GRAPHICS_SOURCES:%.fig=%.pstex)

THREEPOLY_SOURCES=Makefile $(MAINTEXFILE).tex $(THREEPOLY_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	SLII-mathematika.aux 3poly-alco.bib

THREEPOLY_STYLES = cedram-alco.cls amsplain-ac.bst

THREEPOLY_GRAPHICS=$(THREEPOLY_GENERATED_GRAPHICS)							\
	mirage1.eps mirage1-eps-converted-to.pdf							\
	mirage2sanssommets.eps mirage2sanssommets-eps-converted-to.pdf					\
	mirage3.eps mirage3-eps-converted-to.pdf							\
	mirage2sliced.eps mirage2sliced-eps-converted-to.pdf						\
	rectangle-irrationnel-basis.eps rectangle-irrationnel-basis-eps-converted-to.pdf		\
	rectangle-irrationnel.eps rectangle-irrationnel-eps-converted-to.pdf				\
	mirage2.eps mirage2-eps-converted-to.pdf							\
	parametricdim2chambers.eps parametricdim2chambers-eps-converted-to.pdf				\
	BrianchonGramContinu-2.eps BrianchonGramContinu-2-eps-converted-to.pdf				\
	BrianchonGramContinu.eps BrianchonGramContinu-eps-converted-to.pdf				\
	SlicedDilatedtetra0-1.eps SlicedDilatedtetra0-1-eps-converted-to.pdf				\
	SlicedDilatedtetra1-2.eps SlicedDilatedtetra1-2-eps-converted-to.pdf				\
	SlicedDilatedtetra-irrational0-1.eps SlicedDilatedtetra-irrational0-1-eps-converted-to.pdf	\
	SlicedDilatedtetra-irrational1-2.eps SlicedDilatedtetra-irrational1-2-eps-converted-to.pdf	\
	minkowski11.eps minkowski11-eps-converted-to.pdf						\
	minkowski51.eps minkowski51-eps-converted-to.pdf						\
	marsplus.eps marsplus-eps-converted-to.pdf							\
	demimars.eps demimars-eps-converted-to.pdf							\
	pic-en-dim2-barvinok.eps pic-en-dim2-barvinok-eps-converted-to.pdf				\
	pic-en-dim2-conebycone.eps pic-en-dim2-conebycone-eps-converted-to.pdf				\
	conebycone-simplexDim3v3.eps conebycone-simplexDim3v3-eps-converted-to.pdf			\
	fullbarvinok-simplexDim3v3.eps fullbarvinok-simplexDim3v3-eps-converted-to.pdf

### Not used:
## conebycone-simplexDim3004-eps-converted-to.pdf
## fullbarvinok-simplexDim3004-eps-converted-to.pdf
## conebycone-simplexDim3041-eps-converted-to.pdf
## fullbarvinok-simplexDim3041-eps-converted-to.pdf
## 2triangles-eps-converted-to.pdf
## 3-Ehrhart-polynomials-Matthias-18mars-notes-Nicole.pdf
## 3-Ehrhart-polynomials-old-comments.pdf
## 3-Ehrhart-polynomials.pdf
## 3polynomials-nicole-07-janvier-2013.pdf
## 3polynomials-nicole-15-janvier-2013.pdf
## Parametric-versus-Partition-polytopes.pdf
## coneCB-eps-converted-to.pdf
## conebycone-simplexDim4-2-eps-converted-to.pdf
## conebycone-simplexDim4-eps-converted-to.pdf
## document-template.pdf
## floor-s-eps-converted-to.pdf
## floorss-eps-converted-to.pdf
## fullbarvinok-simplexDim3variante.pdf
## fullbarvinok-simplexDim4-eps-converted-to.pdf
## fullbarvinok-simplexDim4variante.pdf
## irrational-tetragon-intro-eps-converted-to.pdf
## pic-en-dim2.mieux.pdf
## randomdim3barvinok.pdf
## randomdim3conebycone.pdf
## square-eps-converted-to.pdf
## tetragon-eps-converted-to.pdf
## tetragon-triangle-eps-converted-to.pdf
## trianglebarvinok.pdf
## unseen-peak-eps-converted-to.pdf


BIB=3poly-alco.bib

.PHONY: figures

figures: $(THREEPOLY_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(THREEPOLY_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

THREEPOLY_SOURCES_AND_MORE=$(THREEPOLY_SOURCES) $(THREEPOLY_GRAPHICS) $(THREEPOLY_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(THREEPOLY_SOURCES)					\
		$(THREEPOLY_GRAPHICS)					\
		$(THREEPOLY_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

clean: 
	-rm -f *.bak *.aux *.log *.bbl *.blg $(THREEPOLY_GENERATED_GRAPHICS)


